A collision model for DNS with ellipsoidal particles in viscous fluid

The article proposes an algorithm to model the collision between arbitrary ellipsoids in viscous fluid. It is composed of several steps, each improving upon the standard procedure employed in the current literature. First, an efficient contact detection algorithm is presented. Then, the semi-implicit Immersed Boundary Method of Tschisgale et al. (2018) is enhanced by the collision forces using the hard-sphere approach, so that the resulting model accounts for fluid forces throughout the entire collision process. Additionally, a new lubrication model is proposed that applies a constant lubrication force in the region where hydrodynamic forces are not resolved by the spatial grid. The new collision model is validated against benchmark test cases of particle wall collisions with excellent agreement. Furthermore, the collision of an ellipsoidal particle with a wall is investigated. The normal restitution coefficient in the case of ellipsoidal particles does not solely depend upon the Stokes number as in the case of spherical particles but is also a function of its shape, and the orientation before the collision. Using the new model, the effect of these parameters on the rebound trajectory is studied. It is found that the maximum normal restitution coefficient decreases significantly as the flatness of the particle increases. Also, the coefficient of restitution depends on the particle orientation, a tendency increasing with particle flatness. >>>>>>>>>>>>>>> Note, that the distance algorithm described in the paper is subject of a Corrigendum: https://www.sciencedirect.com/science/article/pii/S0301932222000313/pdfft?md5=1c1b8e790efdc6785c47297d89906fe6&pid=1-s2.0-S0301932222000313-main.pdf <<<<<<<<<<<<<<<

==> Nomenclature.tex <==
\newcommand{\Units}[1]{\hfill\makebox[4em]{#1\hfill}\ignorespaces}

\newcommand{\DefinitionCol}[1]{\hfill\parbox[t]{12em}{#1}\ignorespaces}

\newcommand{\nomsubtitle}[1]{\item[\bfseries #1]}

\renewcommand\nomgroup[1]{\def\nomtemp{\csname nomstart#1\endcsname}\nomtemp}

\newcommand{\nomstartR}{\nomsubtitle{Roman Symbols}%
	\item[\bfseries Symbol]%
	\textbf{Description}\Units{\textbf{Units}}}
\newcommand{\nomstartG}{\nomsubtitle{Greek Symbols}%
	\item[\bfseries Symbol]%
	\textbf{Description}\Units{\textbf{Units}}}
\newcommand{\nomstartD}{\nomsubtitle{Dimensionless Numbers}%
	\item[\bfseries Symbol]\textbf{Description}\DefinitionCol{\textbf{Definition}}}
\newcommand{\nomstartO}{\nomsubtitle{Other Symbols}%
	\item[\bfseries Symbol]%
	\textbf{Description}}

\renewcommand*{\nompreamble}{\markboth{\nomname}{\nomname}}
%
\newcommand{\nomdescr}[1]{\parbox[t]{0.8\linewidth}{\RaggedRight #1}}
\newcommand{\nomdescrdef}[1]{\parbox[t]{0.5\linewidth}{\RaggedRight #1}}
\newcommand{\nomwithdim}[4]{\nomenclature[#1]{#2}%
	{\nomdescr{#3}\Units{#4}}}
\newcommand{\nomtypeR}[4][]{\nomwithdim{R#1}{#2}{#3}{#4}}
\newcommand{\nomtypeG}[4][]{\nomwithdim{G#1}{#2}{#3}{#4}}
\newcommand{\nomtypeD}[4][]{\nomenclature[D#1]{#2}{\nomdescrdef{#3}\DefinitionCol{#4}}}
\newcommand{\nomtypeO}[3][]{\nomenclature[O#1]{#2}{\nomdescr{#3}}}

%
%\makenomenclature


% -----------------------------------------

%\renewcommand\nomgroup[1]{%
%	\item[\bfseries
%	\ifstrequal{#1}{R}{Roman symbols}{%
%	\ifstrequal{#1}{G}{Greek symbols}{%
%	\ifstrequal{#1}{O}{Other Symbols}{}}}%
%	]}
% -----------------------------------------
\makenomenclature
% variables in the governing equations (Navier-stokes equation)
\nomtypeR[]{$\vec{u}$}{velocity vector, $\vec{u}=(u,v,w)^{T}$}{\si{m/s}}
\nomtypeG[]{$\Omega$}{computational domain}{-}
\nomtypeG[]{$\Omega^\mathrm{f}$}{fluid domain}{-}
\nomtypeG[]{$\Omega^\mathrm{p}$}{particle interior}{-}
\nomtypeR[]{$p$}{pressure}{\si{N/m^2}}
\nomtypeG[]{$\rho_{\mathrm{f}}$}{density of fluid}{\si{kg/m^3}}
\nomtypeG[]{$t$}{time}{\si{s}}
\nomtypeR[]{$\vec{f}_\mathrm{IBM}$}{coupling force imposed to take into account the particle-fluid interaction}{\si{N}}
\nomtypeR[]{$\vec{f}_\mathrm{v}$}{volume force applied to drive the flow}{\si{N}}
\nomtypeG[]{$\boldsymbol{\tau}$}{hydrodynamic stress tensor}{\si{N/m^2}}
\nomtypeG[]{$\mu_\mathrm{f}$}{dynamic viscosity of fluid}{\si{kg/ms}}
\nomtypeR[]{$\vec{\mathbb{I}}$}{identity matrix, $\vec{\mathbb{I}} = \text{diag}(1,1,1)$}{1}
\nomtypeR[]{$x, y, z$}{streamwise, wall-normal, and spanwise coordinates }{\si{m}}
\nomtypeO[]{$\vec{a}\otimes\vec{b}$}{tensor-product of two vectors $\vec{a}$ and $\vec{b}$}
\nomtypeO[]{$\nabla\cdot\vec{A}$}{divergence of a tensor field $\vec{A}$}

% Equation of motion of disperse phase
\nomtypeR[]{$\vec{u}_\mathrm{p}$}{velocity vector, $\vec{u}_\mathrm{p}=(u_\mathrm{p},v_\mathrm{p},w_\mathrm{p})^{T}$}{\si{m/s}}
\nomtypeR[]{$V_\p$}{volume of an ellipsoid}{\si{m^3}}
\nomtypeG[]{$\rho_\p$}{particle density}{\si{kg/m^3}}
\nomtypeR[]{$m_\p$}{mass of an ellipsoid}{\si{kg}}
\nomtypeR[]{$\textbf{n}$}{outward-pointing surface normal vector}{1}
\nomtypeR[]{$\textbf{g}$}{gravitational acceleration}{\si{m/s^2}}

\nomtypeR[]{$L_{\mathrm{x}}, L_{\mathrm{y}}, L_{\mathrm{z}}$}{computational domain length in streamwise, wall-normal, and spanwise direction}{\si{m}}
\nomtypeR[]{$N_{\mathrm{x}}, N_{\mathrm{y}}, N_{\mathrm{z}}$}{number of grid cells in streamwise, wall-normal, and spanwise direction}{\si{1}}
\nomtypeR[]{$N_{\mathrm{p,mob}}$}{number of mobile particles}{1}
\nomtypeR[]{$N_{\mathrm{p,fix}}$}{number of fixed particles}{1}
\nomtypeR[]{$N_{\mathrm{p}}$}{number of particles}{1}
\nomtypeR[]{$H$}{height of the channel}{\si{m}}
\nomtypeR[]{$D_{\mathrm{eq}}$}{volumetrically equivalent diameter of an ellipsoid}{\si{m}}
\nomtypeD[]{$D_{\mathrm{eq}}^+$}{Reynolds number based on friction velocity and particle equivalent diameter}{$\displaystyle \frac{u_\tau D_\mathrm{eq}}{\nu}$}
\nomtypeD[]{$\mathit{Re}_{\mathrm{b}}$}{Reynolds number based on bulk velocity and channel height}{$\displaystyle \frac{U_\mathrm{b} H}{\nu}$}
\nomtypeD[]{$\mathit{Re}_{\mathrm{\tau}}$}{Reynolds number based on friction velocity and channel height}{$\displaystyle \frac{u_\tau H}{\nu}$}
\nomtypeD[]{$\Delta x^+$}{Reynolds number based on friction velocity and grid cell size}{$\displaystyle \frac{u_\tau \Delta_x}{\nu}$}
\nomtypeG[]{$\Delta x, \Delta y, \Delta z$}{computational grid cell size in streamwise, wall-normal, and spanwise direction }{\si{m}}

\nomtypeG[]{$\rho_{\mathrm{p}}$}{density of particle}{\si{kg/m^3}}
\nomtypeG[]{$\vartheta$}{polar angle}{1}
\nomtypeG[]{$\varphi$}{azimuthal angle in the $x$-$y$ plane}{1}
\nomtypeD[]{$\mathit{Fr}$}{Froude number}{$\displaystyle \frac{U_\mathrm{b}}{gH}$}
\nomtypeD[]{$\mathit{Sh}$}{Shields number}{$\displaystyle \frac{u^2_\tau}{\rho'gD_\mathrm{eq}} = \frac{\tau_w}{(\rho_\mathrm{p}-\rho_\mathrm{f})gD_\mathrm{eq}}$}

\nomtypeR[]{$a, b, c$}{longest, intermediate, and smallest axis of an ellipsoid}{\si{m}}
\nomtypeG[]{$\psi$}{sphericity}{1}
\nomtypeG[]{$\mu_{\mathrm{c}}$}{coefficient of static friction}{1}
\nomtypeG[]{$\mu_{\mathrm{d}}$}{coefficient of dynamic friction}{1}
%\nomtypeG[]{$\mu_{\mathrm{r}}$}{coefficient of rolling friction}{1}
%\nomtypeG[]{$\mu_{\mathrm{s}}$}{coefficient of spinning friction}{1}
\nomtypeR[]{$e$}{coefficient of restitution}{1}
\nomtypeG[]{$\nu$}{kinematic viscosity of fluid}{\si{m^2/s}}
\nomtypeR[]{$U_{\mathrm{b}}$}{bulk velocity}{\si{m/s}}
%%
\nomtypeR[]{$V_{\mathrm{t}}$}{total volume of solid phase}{\si{m^3}}
\nomtypeR[]{$V_{\mathrm{i}}$}{volume of particles with an equivalent diameter $i$}{\si{m^3}}
\nomtypeR[]{$V_{\mathrm{s,i}}$}{volume of particles of shape $s$ with an equivalent diameter $i$}{\si{m^3}}

\printnomenclature

